Hierarchical clustering: visualization, feature importance and model selection

We propose methods for the analysis of hierarchical clustering that fully use the multi-resolution structure provided by a dendrogram. Specifically, we propose a loss for choosing between clustering methods, a feature importance score and a graphical tool for visualizing the segmentation of features in a dendrogram. Current approaches to these tasks lead to loss of information since they require the user to generate a single partition of the instances by cutting the dendrogram at a specified level. Our proposed methods, instead, use the full structure of the dendrogram. The key insight behind the proposed methods is to view a dendrogram as a phylogeny. This analogy permits the assignment of a feature value to each internal node of a tree through an evolutionary model. Real and simulated datasets provide evidence that our proposed framework has desirable outcomes and gives more insights than state-of-art approaches. We provide an R package that implements our methods.

==> sections/06-conclusion.tex <==
\section{Final Remarks}
\label{sec:remarks}

We developed a novel paradigm for hierarchical clustering analysis. This framework 
allows the practitioner to choose between clustering algorithms, to interpret the resulting dendrograms, and  to
measure the importance of each feature. Contrary to existing approaches, this is done without losing the rich multi-resolution structure provided by the dendrograms. Indeed, our experiments show that our framework leads to easier-to-interpret and more accurate inference than competing approaches.

Our paradigm is based on 
viewing a dendrogram as a phylogeny. 
This connection opens possibilities that go beyond this work; 
hierarchical clustering analysis may now be 
 enriched with
 other tools
 developed for phylogenetic analyses. 
 %Thus, this work brings up a new study topic regarding hierarchical clustering analysis assisted by phylogenetic methods, with several topics open to discussion and exploration.
 The cross-validated loss, the importance score, and the evolutionary dendrogram are implemented in R  at \url{https://github.com/Monoxido45/PhyloHclust}.
